Data Diversity Matters for Robust Instruction Tuning

Recent works have shown that by curating high quality and diverse instruction tuning datasets, we can significantly improve instruction-following capabilities. However, creating such datasets is difficult and most works rely on manual curation or proprietary language models. Automatic data curation is difficult as it is still not clear how we can define diversity for instruction tuning, how diversity and quality depend on one other, and how we can optimize dataset quality and diversity. To resolve these issue, we propose a new algorithm, Quality-Diversity Instruction Tuning (QDIT). QDIT provides a simple method to simultaneously control dataset diversity and quality, allowing us to conduct an in-depth study on the effect of diversity and quality on instruction tuning performance. From this study we draw two key insights (1) there is a natural tradeoff between data diversity and quality and (2) increasing data diversity significantly improves the worst case instruction following performance, therefore improving robustness. We validate the performance of QDIT on several large scale instruction tuning datasets, where we find it can substantially improve worst and average case performance compared to quality-driven data selection.

==> source_files/experiments.tex <==
We first analyze how the QDIT algorithm affects dataset quality and diversity and then present our main results and analysis.

\subsection{Preliminary Analysis}
To verify that QDIT can indeed control the quality and diversity of the selected dataset, we first investigate whether the facility location function is aligned with our intuitive understanding of diversity. Next, we study how the $\alpha$ parameter affects the dataset's quality and diversity. For this analysis, we apply the QDIT algorithm to the Alpaca dataset \citep{alpaca}.

To qualitatively verify that the facility location function is aligned with dataset diversity, we use the Berkeley Neural Parser \citep{kitaev-klein-2018-constituency, kitaev-etal-2019-multilingual} to extract the root verb and first direct noun from each instruction in the Alpaca dataset. We then plot the distribution of verb-noun pairs in Figure \ref{fig:verb} for random, quality driven, and QDIT data selection. From Figure \ref{fig:verb}, we observe that selecting based on the facility location function indeed improves the dataset diversity compared to random selection, while selecting based on quality alone decreases dataset diversity.

\begin{figure*}
    \centering
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[height=1.8in]{figures/verb_random.png}
        \caption{Random Selection}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[height=1.8in]{figures/verb_quality.png}
        \caption{Quality Driven Selection}
    \end{subfigure}%
    \begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[height=1.8in]{figures/verb_facloc.png}
        \caption{QDIT ($\alpha = 0$)}
    \end{subfigure}%
    \caption{Distribution of root verbs and first nouns selected by different algorithms. The dataset size is 3000.}
    \label{fig:verb}
\end{figure*}

Next we plot how $\alpha$ in QDIT affects dataset quality and diversity in Figure \ref{fig:tradeoff}. Similar figures for other datasets can be found in Appendix \ref{app:tradeoff}. From these figures, we can observe that there is a tradeoff between quality and diversity, and that QDIT allows us to smoothly control this tradeoff. Moreover, we observe that QDIT is able to improve diversity without significantly decreasing data quality. Altogether, these results indicate that QDIT is a practical way to control dataset diversity and quality. 

\begin{figure*}
    \centering
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[height=2.1in]{figures/tradeoff_3k.png}
        \caption{3K Selected Points}
    \end{subfigure}%
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[height=2.1in]{figures/tradeoff_9k.png}
        \caption{9K Selected Points}
    \end{subfigure}%
    \caption{Effect of $\alpha$ on dataset quality and diversity. The red line represents a randomly selected dataset.}
    \label{fig:tradeoff}
\end{figure*}

\subsection{Experimental Setup}
Now that we can control quality and diversity with QDIT, we seek to study how dataset quality and diversity affect instruction following ability.

$\diamond$ \textbf{Training Setup.} We use QDIT on four instruction tuning datasets: Alpaca 52K \citep{alpaca}, Ultrachat 1.3M \citep{ding2023enhancing}, LMSYS-Chat 1M \citep{zheng2023lmsyschat1m}, and a combined dataset of Alpaca 52K, Dolly 15K \citep{DatabricksBlog2023DollyV2}, and the OIG-small-chip2 dataset (210K). We refer to this dataset as ``Mixed 270K". For each dataset we consider two settings: a small data setting and a large data setting. For our main experiments we follow the training procedure from \citet{alpaca} and use LLaMA-1 7B as our base model \citep{touvron2023llama}. In all settings we use the same number of training epochs, meaning that the training cost is proportional to the number of training instructions. Complete hyperparameter details can be found in Appendix \ref{app:hyperparam}.

$\diamond$ \textbf{Evaluation.} We evaluate the trained models in two main ways: through AlpacaFarm \citep{dubois2023alpacafarm} and by using a reward model. For AlpacaFarm, we  evaluate the trained model versus a variety of reference models, employing Claude 2 as the judge on five evaluation sets: InstructEval \citep{wang2022self}, WizardLM \citep{xu2023wizardlm}, Vicuna \citep{vicuna2023}, Koala \citep{koala_blogpost_2023}, and a set of 200 examples manually curated from the ShareGPT dataset. In order to mitigate the effects of the judge LLM's positional bias, we evaluate the responses in both orders (i.e. QDIT response shown first and QDIT response shown second). We then follow \citet{chen2023alpagasus} and measure performance according to winning score ($\frac{\textrm{\# Win} - \textrm{\# Lose}}{\textrm{Total comparisons}} + 1$). Detailed comparison plots can be found in Appendix \ref{app:comprehensive}. In addition to language model based evaluation, we evaluate our models based on the reward score achieved on each evaluation dataset. We use the reward model from \citet{dong2023raft}, which is trained on the Anthropic Helpful Harmless dataset and achieves a test accuracy of over 75\%. We refer to this score as ``HH Score"

$\diamond$ \textbf{Evaluating Robustness.} Beyond evaluating average performance on the test dataset, we also evaluate the worst and best case performance of each model. We can evaluate the worst case performance with the HH Score by calculating the average score achieved on the worst 10\% of instructions for each model (note that the worst instructions can change depending on the model). Similarly, we can evaluate the worst case performance with AlpacaFarm by measuring the losing rate on the worst 40\% (smaller percents reduce the test set size by too much) of instruction categories in the WizardLM evaluation set. Here we use losing rate as a metric because a high losing rate will indicate low robustness. Best case performance is measured in a similar manner with win rate. Measuring best and worst case performance provides more detailed insights into how diversity and quality affect model robustness. 

$\diamond$ \textbf{Baselines.} We primarily compare the QDIT algorithm with two baselines: random data selection and quality based selection. We remark that for the Alpaca dataset instruction-response quality is measured according to ChatGPT (using the same setup as \citet{chen2023alpagasus}) and for all other datasets quality is measured with the previously mentioned reward model.

We also introduce two variants of the QDIT algorithm that attempt to improve data quality and diversity. The first variant, QDIT:Threshold, first orders the data point by quality, and then iteratively selects instructions that do not have a similarity score greater than $\tau$ with any point included selected subset. This algorithm is different from QDIT in that it prevents the dataset from having similar datapoints, which QDIT allows. The second variant we propose is QDIT-Cluster, in which we first cluster the instructions and then select an equal amount of datapoints from each cluster in a quality-driven manner. Comprehensive details can be found in Appendix \ref{app:variants}, where we also provide an analysis of how these algorithms select data.

\begin{table}[!htb]
\caption{Instruction Tuning Results. Random 50K refers to a model trained on a randomly sampled set of 50K points on the corresponding dataset. The top and bottom 40\% win and lose rate is computed on the WizardLM evaluation set.}
% \tiny
\label{tab:main}
\begin{center}
\scalebox{0.68}{
\begin{tabular}{| c | c c c | c  c | c  c |}
\hline
\textbf{Alpaca 52K} & \multicolumn{3}{ c |}{\textbf{Average Performance}} & \multicolumn{2}{ c |}{\textbf{Worst Case Performance}} & \multicolumn{2}{ c |}{\textbf{Best Case Performance}}  \\ 
\cline{2-8}
& \makecell{ \textbf{Winning Score} \\ \textbf{vs. Alpaca 52K $\uparrow$} } & \makecell{ \textbf{Winning Score} \\ \textbf{vs. Random 50K $\uparrow$} } & \makecell{ \textbf{HH Score} \\ \textbf{Mean $\uparrow$} } & \makecell{ \textbf{Bottom 10\%} \\ \textbf{HH Score $\uparrow$} } & \makecell{ \textbf{Bottom 40\%} \\ \textbf{Lose Rate $\downarrow$} } & \makecell{ \textbf{Top 10\%} \\ \textbf{HH Score$\uparrow$} } & \makecell{ \textbf{Top 40\%} \\ \textbf{Win Rate $\uparrow$} }  \\
\hline

Random 9K & 0.975 & - & 3.756 & 0.489 & \textbf{19.23} & 6.942 & 21.77 \\ 
Quality 9K & \textbf{1.013} & - & \textbf{3.944} & \textbf{0.59} & 30.38 & \textbf{7.478} & \textbf{31.82} \\
QDIT 9K & \textbf{1.013} & - & 3.922 & 0.573 & 29.55 & 7.437 & 25.71 \\ \hline
Random 3K & 0.928 & - & 3.601 & 0.368 & 37.35 & 6.876 & 26.25 \\ 
Quality 3K & 0.923 & - & 3.732 & 0.352 & 30.63 & 6.972 & 20.45 \\ \hdashline[1pt/1pt]
QDIT:Cluster 3K & \textbf{0.995} & - & \textbf{3.874} & \textbf{0.601} & 
\textbf{21.98} & 7.025 & \textbf{29.63} \\ 
QDIT:Threshold 3K & 0.986 & - & 3.745 & 0.452 & 25.99 & 6.943 & 29 \\ 
QDIT 3K & 0.961 & - & 3.809 & 0.5 & 25 & \textbf{7.03} & 27.06 \\ \hline \hline
\textbf{Mixed 270K} & \multicolumn{3}{ c |}{\textbf{Average Performance}} & \multicolumn{2}{ c |}{\textbf{Worst Case Performance}} & \multicolumn{2}{ c |}{\textbf{Best Case Performance}}  \\ 
\cline{2-8}
& \makecell{ \textbf{Winning Score} \\ \textbf{vs. Alpaca 52K $\uparrow$} } & \makecell{ \textbf{Winning Score} \\ \textbf{vs. Random 50K $\uparrow$} } & \makecell{ \textbf{HH Score} \\ \textbf{Mean $\uparrow$} } & \makecell{ \textbf{Bottom 10\%} \\ \textbf{HH Score $\uparrow$} } & \makecell{ \textbf{Bottom 40\%} \\ \textbf{Lose Rate $\downarrow$} } & \makecell{ \textbf{Top 10\%} \\ \textbf{HH Score$\uparrow$} } & \makecell{ \textbf{Top 40\%} \\ \textbf{Win Rate $\uparrow$} }  \\
\hline

Random 50K & 0.927 & 1 & 3.6 & 0.396 & \textbf{29.06} & 7.002 & 25.89 \\ 
Quality 50K & 0.973 & \textbf{1.065} & 4.295 & 1.186 & 34.78 & 7.746 & \textbf{28.7} \\
QDIT 50K & \textbf{0.975} & 1.051 & \textbf{4.33} & \textbf{1.223} & 35.22 & \textbf{7.761} & 26.32 \\ \hline
Random 10K & 0.896 & 0.985 & 3.609 & 0.314 & 32.69 & 6.863 & 24.1 \\ 
Quality 10K & 0.956 & 1.042 & 4.342 & 1.117 & 33.33 & 7.952 & 30 \\ \hdashline[1pt/1pt]
QDIT:Cluster 10K & 0.962 & 1.035 & 4.408 & 1.157 & 37.74 & 7.842 & 30.61 \\ 
QDIT:Threshold 10K & 0.98 & 1.06 & 4.282 & 1.051 & 33.96 & 8.005 & \textbf{30.7} \\ 
QDIT 10K & \textbf{0.982} & \textbf{1.063} & \textbf{4.429} & \textbf{1.3} & \textbf{32.65} & \textbf{8.006} & 26.74 \\ \hline \hline

\textbf{Ultrachat 1.3M} & \multicolumn{3}{ c |}{\textbf{Average Performance}} & \multicolumn{2}{ c |}{\textbf{Worst Case Performance}} & \multicolumn{2}{ c |}{\textbf{Best Case Performance}}  \\ 
\cline{2-8}
& \makecell{ \textbf{Winning Score} \\ \textbf{vs. Alpaca 52K $\uparrow$} } & \makecell{ \textbf{Winning Score} \\ \textbf{vs. Random 50K $\uparrow$} } & \makecell{ \textbf{HH Score} \\ \textbf{Mean $\uparrow$} } & \makecell{ \textbf{Bottom 10\%} \\ \textbf{HH Score $\uparrow$} } & \makecell{ \textbf{Bottom 40\%} \\ \textbf{Lose Rate $\downarrow$} } & \makecell{ \textbf{Top 10\%} \\ \textbf{HH Score$\uparrow$} } & \makecell{ \textbf{Top 40\%} \\ \textbf{Win Rate $\uparrow$} }  \\
\hline

Random 50K & 1.189 & 1 & 4.866 & 0.811 & 25 & 8.594 & 50 \\ 
Quality 50K & 1.249 & 1.068 & \textbf{5.91} & 2.116 & \textbf{21.65} & 9.562 & 56.25 \\
QDIT 50K & \textbf{1.26} & \textbf{1.094} & 5.909 & \textbf{2.185} & 22.52 & \textbf{9.69} & \textbf{57.45} \\ \hline
Random 10K & 1.137 & 0.968 & 4.891 & 0.931 & 27.47 & 8.756 & 47.78 \\ 
Quality 10K & 1.228 & 1.011 & 5.844 & 1.846 & 25.47 & \textbf{9.74} & 48.15 \\ \hdashline[1pt/1pt]
QDIT:Cluster 10K & \textbf{1.254} & 1.036 & 5.802 & 1.808 & 20.68  & 9.52 & 51.04 \\ 
QDIT:Threshold 10K & 1.242 & \textbf{1.037} & 5.734 & 1.937 & \textbf{19.64} & 9.64 & \textbf{57.73} \\ 
QDIT 10K   & 1.243& \textbf{1.037} & \textbf{5.849} & \textbf{2.044} & 23.89 & 9.619 & 51.19\\ \hline \hline

\textbf{LMSYS 1M} & \multicolumn{3}{ c |}{\textbf{Average Performance}} & \multicolumn{2}{ c |}{\textbf{Worst Case Performance}} & \multicolumn{2}{ c |}{\textbf{Best Case Performance}}  \\ 
\cline{2-8}
& \makecell{ \textbf{Winning Score} \\ \textbf{vs. Alpaca 52K $\uparrow$} } & \makecell{ \textbf{Winning Score} \\ \textbf{vs. Random 50K $\uparrow$} } & \makecell{ \textbf{HH Score} \\ \textbf{Mean $\uparrow$} } & \makecell{ \textbf{Bottom 10\%} \\ \textbf{HH Score $\uparrow$} } & \makecell{ \textbf{Bottom 40\%} \\ \textbf{Lose Rate $\downarrow$} } & \makecell{ \textbf{Top 10\%} \\ \textbf{HH Score$\uparrow$} } & \makecell{ \textbf{Top 40\%} \\ \textbf{Win Rate $\uparrow$} }  \\
\hline

Random 50K & 1.093 & 1 & 4.791 & 0.958 & 32.35 & 8.629 & 44.21 \\ 
Quality 50K & \textbf{1.22} & \textbf{1.182} & 5.963 & 2.133 & \textbf{30} & 9.361& \textbf{53.06} \\
QDIT 50K & 1.217 & 1.168 & \textbf{6.074} & \textbf{2.278} & 34.48 & \textbf{9.484} & 51.55\\ \hline
Random 10K & 1.108 & 1.002 & 4.906 & 0.981 & 26.21 & 8.67 & 44.66 \\ 
Quality 10K & 1.191 & 1.135 & \textbf{6.139} & 2.335 & 31.58 & 9.69 & 48.28 \\ \hdashline[1pt/1pt]
QDIT:Cluster 10K & 1.218 & 1.143 & 6.125 & 2.085 & 28.44 & \textbf{9.787} & 51.02 \\ 
QDIT:Threshold 10K& \textbf{1.22} & \textbf{1.173} & 5.978 & 2.319 & 26.13 & 9.709 & \textbf{55.42} \\ 
QDIT 10K& 1.217 & 1.142 & 6.078 & \textbf{2.465} & \textbf{25.53} & 9.712 & 52.5 \\ \hline

\end{tabular}}
\end{center}
\end{table}

\subsection{Main Results}
The main experimental results can be found in Table \ref{tab:main}. We mainly focus our analysis on the low data settings, as we find models trained with QDIT can match or beat the models trained in the high data settings while significantly reducing training cost. Nonetheless, we include the high data setting for reference.

\textbf{Effect of Quality.}  Similar to prior works, we find that selecting data based on quality significantly improves average performance, improving the winning score versus Alpaca 52K by 5.41\% and the average HH score by 17.14\% in low data settings. However, we also find that selecting based on quality alone can hurt worst case performance, increasing the bottom 40\% losing rate in two out of four settings compared to random data selection. We hypothesize that this performance drop is due to the fact that quality based selection hurts dataset diversity.

\textbf{Effect of Diversity.} On the other hand, we find that data selection with QDIT is able to achieve both a high average HH score (QDIT improves upon quality driven selection by 2.56\% for winning score vs Alpaca 52K and improves average HH score by 1.29\% in low data settings) while achieving a much better worst case performance than both random and quality-driven selection. In particular, we find that QDIT improves worst case HH score by 18.68 \% and decreases worst case losing rate vs Alpaca 52K by 11.45\% when compared to quality-driven data selection. We suspect that QDIT's more diverse dataset teaches the model to a respond to a wide range of instructions, therefore decreasing the probability that it fails to follow evaluation instructions. We find that QDIT can also maintain best case performance when compared to quality-diven selection, as the best case HH score is improved by 0.12\%. From these experiments we conclude that by increasing data diversity while maintaining data quality, QDIT can improve robust instruction following capability.
% . However, improvements in worst case performance are typically more important than improvements in best case performance, as improving robustness will result in a more consistent and user friendly model. 
% Finally, we find that models trained trained in the low data setting with QDIT can match or outperform quality-driven data selection with 3 to 5 times larger budget, therefore greatly reducing  training cost.

\textbf{QDIT Variants.} We also observe that the two variants of QDIT can improve average performance compared to random data selection, but they do not necessarily improve worst case performance compared to quality based selection. Our experiments suggest that clustering based data selection is highly sensitive to the performance of the clustering algorithm. For example, clustering may be easy on datasets like Alpaca which are derived from a small set of seed tasks, but difficult for larger and human generated instructions like LMSYS. For threshold based selection, we hypothesize that constraining intra-datapoint similarity is not as important as selecting instructions that cover the entire training set.




\subsection{Analysis}

\textbf{Effect of $\alpha$.} We plot the effect of $\alpha$ on average and worst case performance in Figure \ref{fig:alpha}.  From Figure \ref{fig:alpha}, we can see that QDIT is relatively robust to the value of $\alpha$, with values of $\alpha \in \{0.5, 0.7, 0.9\}$ typically having the highest worst case and average performance. However, decreasing $\alpha$ by too much (i.e. $\alpha=0.1$) will result in a significant drop in performance, as will increasing $\alpha$ by too much ($\alpha = 1$). This highlights the need for a careful tradeoff between dataset quality and diversity.

\begin{figure*}
    \centering
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[height=1.4in]{figures/alpaca_alpha.png}
        \caption{Alpaca 3K}
    \end{subfigure}%
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[height=1.4in]{figures/mixed_alpha.png}
        \caption{Mixed 10K}
    \end{subfigure}%
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[height=1.4in]{figures/ultrachat_alpha.png}
        \caption{Ultrachat 10K}
    \end{subfigure}%
    \begin{subfigure}{0.24\textwidth}
        \centering
        \includegraphics[height=1.4in]{figures/lmsys_alpha.png}
        \caption{LMSYS 10K}
    \end{subfigure}%
    \caption{Effect of $\alpha$ on best case and worst case performance. The red line represents a randomly selected dataset. Worst reward refers to the bottom 10 percent of HH scores.}
    \label{fig:alpha}
\end{figure*}

\textbf{Benchmark Performance.} For a more comprehensive evaluation of QDIT, we follow InstructEval \citep{chia2023instructeval} and evaluate our model on various benchmark datasets including MMLU \citep{hendrycks2020measuring}, BBH \citep{suzgun2022challenging}, DROP \citep{dua2019drop}, and HumanEval \citep{chen2021evaluating}. Although these benchmarks are not fully aligned with instruction following performance, we find that QDIT uniformly improves MMLU performance and performs best on BBH and DROP in three out of the four scenarios when compared with quality driven selection. These results further confirm the efficacy of QDIT.


\begin{table}[!h]
\center
\caption{Evaluation on benchmark datasets. We bold the best result out of quality based selection and QDIT based selection. Details can be found in Appendix \ref{app:benchmarks}.}
\label{tab:benchmark}
\scalebox{0.9}{
\begin{tabular}{| c | c c c c | c  c c  c |}
\hline & \multicolumn{4}{ c |}{\textbf{Alpaca 9K}} & \multicolumn{4}{ c |}{\textbf{Mixed 10K}}  \\ 
\cline{2-9}
& MMLU & BBH & DROP & HumanEval & MMLU & BBH & DROP & HumanEval \\
\hline

Random & 34.18 & 31.69 & 26.84 & 8.54 & 32.93 & 30.92 & 20.33 & 10.37 \\ \hdashline[1pt/1pt]
Quality & 34.53 & \textbf{31.17} & 24.57 & \textbf{11.57} & 33.07 & 31.38 & \textbf{26.37} & 10.37 \\
QDIT & \textbf{35.64} & 30.85 & \textbf{26.55} & 7.93 & \textbf{33.29} & \textbf{32.36} & 26.19 & 10.37 \\ \hline
\hline & \multicolumn{4}{ c |}{\textbf{Ultrachat 10K}} & \multicolumn{4}{ c |}{\textbf{LMSYS 10K}}  \\ 
\cline{2-9}
& MMLU & BBH & DROP & HumanEval & MMLU & BBH & DROP & HumanEval \\
\hline

Random & 32.12 & 33.19 & 26.24 &13.41  & 33.05 & 32.57 & 25.06 & 15.85 \\ \hdashline[1pt/1pt]
Quality & 35.44 & 32.06 & 17.01 & 12.2 & 34.74 & 32.32 & 25.95 & 10.36 \\
QDIT & \textbf{35.78} & \textbf{32.66} & \textbf{26.73} & \textbf{13.41} & \textbf{35.9} & \textbf{32.76} & \textbf{26.22} & \textbf{11.58} \\ \hline

\end{tabular}}
\end{table}

\textbf{Different Base Models.} We evaluate the performance of QDIT with different base models in Figure \ref{fig:base}. From Figure \ref{fig:base} we find that QDIT can improve both average performance and worst case performance for other base models, supporting our main results. Interestingly we find that the Mistral model performs best according to HH score, but worst according to AlpacaFarm evaluation \citep{jiang2023mistral}. This highlights the importance of using multiple evaluation strategies.

\begin{figure*}
    \centering
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[height=2.13in]{figures/mistral_results.png}
        \caption{Different Base Models}\label{fig:base}
    \end{subfigure}%
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[height=2.1in]{figures/data_ablation.png}
        \caption{Different Data Sizes (Thousands)}\label{fig:data-able}
    \end{subfigure}%
    \caption{(a) Ablation with different base models. The train set is 10K instructions selected from Ultrachat. (b) Ablation with different data sizes. The worst reward is computed as the bottom 10 percent of HH scores, and the winning score is vs. Alpaca 52K.}
    
\end{figure*}

\textbf{Data Size.} We evaluate the performance of QDIT with different training data sizes in Figure \ref{fig:data-able}, where we find that QDIT results in a 3-4 times improvement in data efficiency (and therefore training cost) as measured by robust performance. We also find that increasing the dataset size beyond $50K$ only results in marginal gains of average performance, and can even decrease worst case HH score. We hypothesize this phenomena is due to overfitting.


\textbf{Case Study.} 
We conduct a case study in Figure \ref{fig:case}. We observe that quality based selection does not select an instruction similar to the test instruction and fails to respond correctly. On the other hand, QDIT does train on a similar instruction due to its more diverse training set and correspondingly responds to the instruction correctly. We remark that in practice the distance to the closest training instruction does not always correlate to evaluation performance, as we find embedding distance may not capture important aspects of an instruction such as the format it is in or the desired response format. In the future, we hope to investigate how different similarity metrics impact QDIT and instruction tuning performance.

\begin{figure*}
    \centering
    \includegraphics[height=3.6in]{figures/case_study.png}
    \caption{Spotify playlist case study.}
    \label{fig:case}
\end{figure*}



==> source_files/intro.tex <==
Large pre-trained language models have demonstrated a remarkable ability to perform a wide range of natural language processing tasks \citep{vaswani2017attention, devlin2018bert, radford2019language, he2020deberta, brown2020language}. Although these models are powerful, pre-trained models such as GPT-3 can be quite difficult to work with and often do not follow user instructions \citep{brown2020language}. To make language models more user-friendly and to unlock instruction-following capabilities, researchers have turned to instruction tuning, in which language models are trained to follow instructions on a small set of example instruction-response pairs \citep{mishra2021cross, wei2021finetuned, sanh2021multitask, wang2022super}. Instruction tuning has become extremely popular, allowing researchers to train powerful and aligned language models with a relatively small budget \citep{alpaca, vicuna2023, xu2023wizardlm}.

One of the main challenges of instruction tuning is selecting the instruction data. Recent works have found that the composition of the instruction-tuning dataset significantly impacts the instruction following ability of the trained model, with most works identifying two qualities that an instruction tuning dataset should have: it should be high quality \citep{chen2023alpagasus, peng2023instruction} and it should cover a wide range of tasks (i.e. be diverse) \citep{wei2021finetuned, zhou2023lima, gudibande2023false}. However, as of yet there has been little study of how these two factors (quality and diversity) affect on one another and how researchers can automatically select high quality and diverse datasets. Instead, current work relies on manual data curation \citep{zhou2023lima} or optimize one quantity only \citep{chen2023alpagasus, peng2023instruction, wang2022self}.

To bridge this gap we introduce a new algorithm, Quality-Diversity Instruction Tuning (QDIT), to select diverse and high quality instruction tuning datasets. QDIT is inspired by submodular optimization \citep{fujishige2005submodular} and works by iteratively selecting the datapoint that will improve the joint quality-diversity score the most. QDIT provides an effective way to control the diversity and quality of the instruction tuning dataset, allowing us to conduct an in-depth study of diversity and quality in instruction tuning. From this study we identify two key findings: (1) there is an inherent tradeoff between dataset diversity and dataset quality and (2) improving dataset diversity primarily improves the worst and average case instruction following ability, while not affecting best case instruction following ability much. Based on these finding, we are able to use QDIT to optimize the quality-diversity tradeoff, improving worst case performance while maintaining or improving best case and average performance for robust instruction following. We extensively validate the QDIT algorithm with experiments on four large scale instruction tuning datasets.

The rest of this article is organized as follows: Section \ref{sec:related-work} covers related literature, Section \ref{sec:method} presents the QDIT algorithm, Section \ref{sec:experiments} contains our experimental results, and Section \ref{sec:conclusion} concludes our work.

==> source_files/method.tex <==
Before presenting QDIT, we discuss how to quantify and optimize dataset diversity.
\subsection{Quantifying Dataset Diversity and Quality}

Given a set $A \subseteq V$, a natural way to measure the diversity of the set $A$ with respect to $V$ is by the facility location function \citep{cornuejols1983uncapicitated}
\begin{align}
\label{eq:div}
    d(A) = \sum_{v \in V} \textrm{max}_{a\in A} sim(a, v)
\end{align}
Intuitively, we can see that a set A that has a high diversity score $d(A)$ will have an element $a \in A$ close to each element $v \in V$ and will therefore be representative of the set $V$.


In order to optimize the facility location function, researchers typically use the greedy data selection algorithm \citep{nemhauser1978analysis}, where the datapoint that most increases the diversity score of the current subset is selected at each iteration. The greedy algorithm is shown in Algorithm \ref{alg:greedy}, where $d(a|A) = d(a\cup A) - d(A)$. We remark that this algorithm achieves the best possible approximation ratio (in the worst case) that a polynomial time algorithm can achieve unless $P=NP$ \citep{nemhauser1978analysis}.

To measure dataset quality, we follow prior works and measure the quality of each (instruction, response) pair using a large language model such as ChatGPT \citep{chen2023alpagasus} or measure the quality of each datapoint using a reward model trained on large amounts of human preference data \citep{ouyang2022training, bai2022constitutional}. We refer to such a function with $q(\cdot)$, and measure a dataset's overall quality by averaging the quality score of each datapoint.

\subsection{Quality-Diversity Instruction-Tuning}
In order to select data based on both quality and diversity, we alter the greedy algorithm so that instead of selecting based on diversity alone at each iteration, we select data based on a linear combination of quality and diversity $(1-\alpha) d(a) + \alpha q(a)$. Here $\alpha$ is a hyperparameter that can be used to control the diversity tradeoff. We remark that when $\alpha = 1$, QDIT becomes the quality driven selection algorithm proposed in \citet{chen2023alpagasus} and when $\alpha = 0$ QDIT becomes the classical greedy algorithm \citep{nemhauser1978analysis}. QDIT will select points that most increase the joint diversity-quality score of the data set, therefore satisfying our goal of building a diverse and high quality dataset. The QDIT algorithm can be found in Algorithm \ref{alg:qdit}. In QDIT, we use the cosine similarity of instruction embeddings as the similarity function in \eqref{eq:div}, where the instruction embeddings are computed with sentence transformers \citep{reimers-2019-sentence-bert}. See appendix \ref{app:sim} for more details.

\begin{minipage}{.45\textwidth}
\begin{algorithm}[H]
\caption{Greedy Data Selection}\label{alg:greedy}
\begin{algorithmic}[1]
\Require $K$ \Comment{Desired subset size} 
\State $A \gets \emptyset$
\State $R \gets V$
\State $N \gets 0$
\While{$N < K$}
    \State $a \gets \textrm{argmax}_{a\in R} d(a|A)$
    \State $A \gets A \cup \{a \}$
    \State $R \gets R \setminus a$
    \State $N \gets N + 1$
\EndWhile
\end{algorithmic}
\end{algorithm}
\end{minipage}%
\hfill
\begin{minipage}{.45\textwidth}
\begin{algorithm}[H]
\caption{QDIT Data Selection}\label{alg:qdit}
\begin{algorithmic}[1]
\Require $K, \alpha$
\State $A \gets \emptyset$
\State $R \gets V$
\State $N \gets 0$
\While{$N < K$}
    \State $a \gets \textrm{argmax}_{a\in R} (1 - \alpha) * d(a|A) + \alpha * q(a)$
    \State $A \gets A \cup \{a\}$
    \State $R \gets R \setminus a$
    \State $N \gets N + 1$
\EndWhile
\end{algorithmic}
\end{algorithm}
\end{minipage}

\textbf{Computational Complexity of QDIT. } Finding $a \in A$ that maximizes the quality-diversity score at each time step has complexity $\cO(|V|^3)$, leading to a total complexity of $\cO(|V|^3K)$ for QDIT based data selection. This is problematic, since for some datasets $|V|$ is greater than 1 million. We take several approaches to reduce data selection cost: (1) parallelization on GPUs, (2) employing the lazy greedy selection algorithm of \citet{minoux2005accelerated}, and (3) sub-sampling according to \citet{mirzasoleiman2015lazier}. These methods can be employed simultaneously, allowing us to select from millions of datapoints within a few hours. We provide more details in Appendix \ref{app:cost}, where we find that data selection has minimal cost when compared to training.



==> source_files/related-work.tex <==

% The first works on instruction tuning constructed instruction tuning datasets from existing NLP datasets, framing each task as instruction following. \citep{wei2021finetuned, sanh2021multitask, mishra2021cross}. Although this lead to remarkable generalization performance on held-out NLP tasks, the responses from the resulting models are typically not in the style of a conversational agent. To train more user-friendly models, recent works have constructed instruction tuning datasets using instructions generated from either human annotators \citep{ouyang2022training, zhou2023lima, DatabricksBlog2023DollyV2, touvron2023llama} or high quality language models \citep{wang2022self, bai2022constitutional, alpaca, vicuna2023, peng2023instruction}. These works typically train on a relatively small set of instructions (i.e. less than 100,000). Notably, LIMA \citep{zhou2023lima} only trains on 1000 instructions, hypothesizing that the composition of the instruction-tuning dataset matters more than the dataset size. 

Given the widespread availability of large instruction tuning datasets \citep{ding2023enhancing, zheng2023lmsys}, a new question has emerged: How should we select a training dataset from existing ones? Here data selection is necessary as training on large scale instruction tuning datasets will have a large cost and result in deterioration of model capabilities \citep{ouyang2022training, zhou2023lima, chen2023alpagasus}. Several strategies have been proposed to answer this question, mainly focusing on improving dataset quality. \citet{li2023quantity} propose to select instructions based on difficulty. \citet{chen2023alpagasus} propose Alpagasus, in which a large language model such as ChatGPT is employed to select the highest quality (instruction, response) pairs from a large dataset. \citet{peng2023instruction} also seek to improve data quality, and do so by rewriting answers to instructions with GPT-4. We seek to improve upon these algorithms by including both diversity and quality in the selection criteria.

Our work is also related to several works that use submodular optimization to increase dataset diversity in natural language processing \citep{kumar2019submodular, kirchhoff2014submodularity}. However, to the best of our knowledge we are the first to include both data quality and diversity in the selection procedure.
